Understanding Differential Search Index for Text Retrieval

The Differentiable Search Index (DSI) is a novel information retrieval (IR) framework that utilizes a differentiable function to generate a sorted list of document identifiers in response to a given query. However, due to the black-box nature of the end-to-end neural architecture, it remains to be understood to what extent DSI possesses the basic indexing and retrieval abilities. To mitigate this gap, in this study, we define and examine three important abilities that a functioning IR framework should possess, namely, exclusivity, completeness, and relevance ordering. Our analytical experimentation shows that while DSI demonstrates proficiency in memorizing the unidirectional mapping from pseudo queries to document identifiers, it falls short in distinguishing relevant documents from random ones, thereby negatively impacting its retrieval effectiveness. To address this issue, we propose a multi-task distillation approach to enhance the retrieval quality without altering the structure of the model and successfully endow it with improved indexing abilities. Through experiments conducted on various datasets, we demonstrate that our proposed method outperforms previous DSI baselines.

==> problem_state.tex <==
\section{Empirical Analysis} \label{EmpAna}
In this section, we conduct an empirical analysis to examine to what extent the DSI framework satisfies the basic requirements as a functioning IR model. Specifically, we summarize \textit{exclusivity}, \textit{completeness}, and \textit{relevance ordering}, as three essential abilities that are required for an IR system with indexing, retrieval, and ranking functionalities, which are later defined in further details. %We consider these three capabilities to be essential for a search framework to be capable of providing users with accurate, comprehensive, and relevant information in a retrieval task. 

%Notations used throughout this paper are summarized in Table\ref{tab:notation}.

%\subsection{Experimental Setup}
%Apart from the DSI-QG model, the classical BM25 [cite] and the more recent TCT-ColBERT are chosen to represent sparse and dense retrieval models respectively in this study.

In order to examine the capabilities of various retrieval paradigms, a controlled experimental study was conducted using three different models: the classical BM25 [cite], the more recent TCT-ColBERT [cite], and DSI-QG [cite]. These models represent distinct approaches to information retrieval, including sparse indexing, dense indexing, and differentiable search indexing, respectively. The experiments are conducted on the widely used MS MARCO Passage dataset. More details about these models can be found in Appendix xxx.

\subsection{Exclusivity}
\begin{figure*}[tbp]
  \centering
  \subfloat[Hits@1 of different retrieval models on fragments of varying lengths and pseudo queries.\label{fig:exclusivity}] {\includegraphics[width=0.3\textwidth]{pics/after_train/exclusivity_after.png}}
 \hfill 	
  \subfloat[Completeness\label{fig:completene}]{\includegraphics[width=0.33\textwidth]{pics/after_train/completeness_after.png}}
 \hfill	
  \subfloat[Relevance\label{fig:relevance}]{\includegraphics[width=0.31\textwidth]{pics/after_train/relevance_after.png}}
\\	
	\caption{Results.}
       \label{fig:analysis}
\end{figure*}
\textbf{Exclusivity: definition} refers to the uniqueness of documents in a search engine, i.e., the one-to-one correspondence between document content and document identifier, which determines the extent to which a retrieval framework can distinguish different documents in a collection. The document representation is expected to retain the uniqueness of the original text as much as possible, thus ensuring the validity and stability of the retrieval results. We formally define exclusivity as a bijective (invertible) function:
\begin{equation}
    d_i \twoheadrightarrow\!\!\!\!\!\!\mapsto id_i, \ \text{for} \  {d_i} \in \mathcal{D}
    \ \text{and} \  {id_i} \in \mathcal{I}
\end{equation}
\noindent where $\twoheadrightarrow\!\!\!\!\!\!\mapsto$ indicates that this function is a one-to-one correspondence between $\mathcal{D}$ and $\mathcal{I}$.
% where $\twoheadrightarrow\!\!\!\!\!\!\mapsto$ is a function that has a unique output for every input in its domain. 
This means that for each individual $d_i$ in $\mathcal{D}$, there is only one document id in the range that the function maps to. Additionally, every $id_i$ in the range must have a corresponding document representation in $\mathcal{D}$.
In actual implementation, the DSI model is only trained for a one-way mapping (i.e., from document representation to document identifier). Therefore, in our analysis, we examine the injective relationship for various models by testing the case of a single directional mapping from a document to its identifier.

\textbf{Exclusivity: Experimental Setup.} 
Both sparse and dense indexes are well-established indexing methods that have been widely and extensively applied. 
% These methods explicitly store each sample in the set in separate entries, ensuring a one-to-one correspondence between document representations and their identifiers. This theoretically guarantees good exclusivity for these methods. 
These methods involve either the storage of statistical information pertaining to the vocabulary of a collection or the compression of each sample within the collection into a vector. The presence of these documents in the index is represented in a manner that enables the storage of unique information about the documents, thus facilitating the establishment of a one-to-one correspondence between the documents and their identifiers by the retrieval framework.
However, differentiable search indexes use model parameters to store all the information in a collection, which makes it difficult to directly observe the exclusivity of the model due to its black-box nature. This presents a challenge in terms of understanding the exclusivity of differentiable search indexes compared to other indexing methods.
To systematically assess the exclusivity of various models, we utilize pre-stored or learned index information as queries for assessing the models. Specifically, we input original document fragments of varying lengths or pseudo-queries derived from the original documents [cite] to the models and assess their capacity to retrieve the corresponding documents as the highest-ranked retrieval outcomes. Following the DSI-QG setup [cite], a series of experiments are conducted utilizing the training set of MS MARCO 100k [cite] to evaluate the exclusivity of various models.
The length of the query extracted from the original document is varied within the set {16, 32, 64, 128} and is extracted from the beginning of the original documents. The pseudo queries are generated by DocT5Query, which was based on the full text of the passage and followed the same procedures as the DSI-QG training data generation process.

\textbf{Exclusivity: Results.}
% Figure~\ref{fig:exclusivity} illustrates the use of the Hits@1 metric to evaluate the capability of various models to recall the correct document id, as the top-ranked result, when utilizing both original text fragments and pseudo-queries as inputs. 
As illustrated in the figure~\ref{fig:exclusivity}, we utilize the Hits@1 metric to evaluate the ability of different models to first recall the original text id when using either original text fragments or pseudo-queries as input.
The results indicate that both the BM25 and TCT-ColBERT models exhibit exceptional performance in accurately recalling the corresponding document id when utilizing original text fragments, with accuracy increasing as the length of the original text increases. Additionally, both models exhibit relatively strong results when applied to unseen pseudo-queries. However, the DSI-QG model, while demonstrating the ability to recall the corresponding document id for pseudo-queries used in its training data, struggles to recall the correct id when applied to the original document. This implies that the effectiveness of the DSI-QG model is limited to the specific pseudo-query and corresponding document id, and may not extend to other original documents. This has important implications for its utility in retrieval tasks, particularly in cases where short pseudo-queries with high repetition and low information content are commonly used.

%Figure\ref{fig:exclusivity} illustrates the utilization of the Hits@1 metric to evaluate the ability of various models to recall the original document id as the top-ranked document when utilizing both original fragments and pseudo-queries as input. Results indicate that both the BM25 and TCT-ColBERT models demonstrate superior performance in accurately recalling the corresponding document id when inputting original fragments, with accuracy increasing as the length of the original text increases. Additionally, both models exhibit relatively strong results when applied to unseen pseudo-queries. However, the DSI-QG model, while being able to recall the corresponding document id for the pseudo-query used in its training data, struggles to recall the corresponding id for the original document. This implies that the effectiveness of DSI-QG is limited to the specific pseudo-query and corresponding document id, and may not extend to the original document. This could have significant implications for its utility in retrieval tasks, given the high repetition and low information content typically associated with short pseudo queries.

\subsection{Completeness}
\textbf{Completeness: Definition} is the ability of an indexing model to retrieve all eligible documents in a collection. This means that if a document has relevant content and meets the search criteria, then that document is expected to appear in the search results. To obtain more comprehensive search results, the index structure needs to store as complete document information as possible (e.g., sparse search indexes) or to maximize the identification and memory of more valuable key document information (e.g., dense search indexes). In this context, the completeness of an index is narrowly defined as its ability to store essential information contained within a document, taking into consideration the various differences in index structures and practical application requirements. Completeness is defined formally as:

 \textbf{Completeness: Experimental Setup.} 
 To determine the completeness of information stored in various indexes, we conduct an experiment in which we randomly select 10k documents from the training set of MS MARCO 100k [cite] and their corresponding user queries. Utilizing the BERT reranker with cross-attention [cite] as a strong relevance weighting model, we identify the most relevant segments of each document by dividing the documents into equal-length chunks with overlaps and calculating the relevance score of each chunk with respect to the user query. 
 It is important to acknowledge that it can be challenging to fully determine all of the key components of a document due to the lack of human annotations. Therefore, it is assumed that the portions of the document that are most relevant to the user query constitute a subset of the document's essential content. This subset, consisting of all document chunks that are most relevant to the user query, is then used as queries in various retrieval models, and their ability to accurately recall the corresponding document is evaluated as a measure of completeness.
 %It should be noted that it is difficult to determine all key aspects of a document through experimental processes, so we assume that the chunks with the highest relevance to the user query represented a portion of the document's key content. That is, we considered the set of all document chunks that are most relevant to the user query to constitute a subset of the document's key content. We then enter the text from this subset as queries in different retrieval models and evaluate their ability to preferentially recall the documents in which they are located as a measure of the completeness of different indexes.
 

 \textbf{Completeness: Results.}
 The results depicted in Figure\ref{fig:completene} demonstrate the efficacy of various retrieval paradigms in identifying key textual information within a document. Both BM25 and TCT-ColBERT exhibit a high probability of accurately returning the corresponding document id, with a probability greater than 95\% when the top result is considered, and surpassing 99\% when the top 10 results are examined. This suggests that both sparse and dense indexing methods effectively retain the crucial content of the original document in relation to the user's query. In contrast, DSI-QG demonstrates a lack of proficiency in identifying the original document id when presented with key content pertaining to the query, indicating that under the current training methodology, the differentiable search index may fail to capture the core information integral to the retrieval task, leading to suboptimal performance for the user.

\subsection{Relevance Ordering}
\textbf{Relevance Ordering} is an essential ability of non-boolean IR models which outputs a sorted list of documents in decreasing order of relevance of the documents to the query. We regard ranking as a partially ordered relationship of all documents in an index relative to a particular user query. For two documents $d_i$ and $d_j$ that both appear in the result list of a one-time retrieval operation $\operatorname{R}(q_t, \operatorname{M})$ on query $q_t$ based on a certain retrieval paradigms $\operatorname{M}$, we formally define Relevance Ordering as:
\begin{align}
    d_j \leq_{q_t} d_i, \ & \text{if}\ \operatorname{s}(q_t, d_j) \leq \operatorname{s}(q_t, d_i), \notag \\ 
    & \text{for} \ \forall d_i, d_j \in R(q_t, \operatorname{M})\; 
\end{align}
where $\operatorname{s}(q_t, d_*)$ is the predicted relevance score of $d_*$, which is in the top-k recall list $(id^1, id^2, ..., id^k)$ given by $\operatorname{R}(q_t, \operatorname{M})$. 

For $d_i$ in the top-k recall list of $\operatorname{R}(q_t, \operatorname{M})$ and $d_o$ in the index pool but not in the top-k result list, we formally define Relevance Ordering as:
\begin{align}
    d_o \leq_{q} d_i,\ & \text{for} \ \forall d_i \in R(q_t, \operatorname{M})\notag \\& \text{and}\;\forall d_o \in \mathcal{D} \setminus R(q_t, \operatorname{M})
\end{align}
where $\mathcal{D} \setminus R(q_t, \operatorname{M})$ is the absolute complement of the set $R(q_t, \operatorname{M})$ in the set $\mathcal{D}$.

\textbf{Experimental Setup.} 
In order to assess the relevance order of text to a given query in the MS MARCO passage dataset, which is characterized by a low level of annotation (typically only one relevant document per query) [cite], we employed the same BERT Reranker as in XXX. To this end, we randomly selected 10k queries from the training set of MS MARCO 100k and used the three retrieval models to predict the top 10 documents for each query. All documents that appear in the result list are included in a set referred to as $\mathcal{S}$. Additionally, we randomly select 10 documents from the dataset for each query, and these randomly selected documents are included in a set referred to as $\mathcal{T}$. The BERT Reranker is then used to evaluate the relevance of the documents in both $\mathcal{S}$ and $\mathcal{T}$ to the corresponding query, and the distribution of the retrieval result orders is analyzed for individual models.
In order to evaluate the performance of a given model, we employ a methodology that involves the following steps. We first ... calculating the average number of random documents that exhibit a higher score than those at each corresponding ranking position within the results returned by the model. It is important to note that, as we assume that none of the random documents are relevant to the query if a significant proportion of these documents exhibit higher scores than those returned by the model, this serves as an indication that the model is returning less relevant documents.
% Specifically, we employed a normalization process for the ranking distribution. For a given query $q$, if there are a total of $r$ document occurrences in the sets $\mathcal{S} \cup \mathcal{T}$, we define the normalized ranking score $rs_d$ for any document $d$ belonging to the set as:
% \begin{equation}
%     rs_d = \frac{k}{r}
% \end{equation}
% where $k$ is the rank of $d$ in the list after scoring by BERT ranker.

\textbf{Results.}
Figure~\ref{fig:relevance} plots the rank positions of the result list (x-axis) against the random confusion scores at each position (y-axis).  
% that as the ranking position of the documents returned by the model lowers, the number of random documents with higher scores also increases. 
This suggests that for the model employed in the experiments, the relevance ordering is largely maintained for documents that are a part of the $R(q, \operatorname{M})$.  
However, in comparison to TCT-ColBERT and BM25, the differentiation of the second-ranked document returned by DSI-QG relative to the random documents diminishes significantly and becomes increasingly indistinguishable as the ranking lowers. By the tenth document in the list returned by DSI-QG, there are approximately four to five random documents that score higher relative to that document, which is indicative of a nearly random distribution. Thus, for the second case of Relevance Ordering, the differentiable search index is found to be inadequate, and the utilization of differentiable search indexing on data with deep annotations, such as TREC DL, may be hindered to a significant extent.
\begin{table}
  \centering
  \caption{Summary of notation.}
  \label{tab:notation}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{@{}l|l@{}}
    \toprule
    \textbf{Symbol} & \textbf{Definition} \\ \midrule
    $\mathcal{D}=\{d_i\}$ & Set of documents stored in the index. \\ [0.8ex]
    $\mathcal{I}=\{id_i\}$ & Set of docIDs of documents in $\mathcal{D}$. \\ [0.8ex]
    $\mathcal{Q}=\{q_i\}$ & Set of user queries. \\ [0.8ex]
    % $\operatorname{Ix}$ & An index of $\mathcal{D}$. \\ [0.8ex] % One-to-one correspondence of $d_i$ and $id_i$. \\ [0.8ex]
    % $\operatorname{DSI}(d) = id$ & Differentiable Search Index \\ [0.8ex]
    $\operatorname{M}(d_i)$ & An index function mapping $d_i$ to $id_i$. \\ [0.8ex]
    $\operatorname{R}(q_i, \operatorname{M})$  & A retrieval operation for $q_i$ based on $\operatorname{M}$. \\ [0.8ex]
    % $(id^1, id^2, ..., id^k)$  & List of retrieval results of $\operatorname{R}(q,\operatorname{M})$. \\ [0.8ex]
    $\operatorname{s}(q_i, d_i) $ & Relevance score of $q_i$ and $d_i$. \\ [0.8ex]
    $d_j \leq_{q} d_i$ & \begin{tabular}[c]{@{}l@{}} A binary relation that $d_i$ is more\\ relevant to $q$ than $d_j$ \end{tabular}\\ \bottomrule
  \end{tabular}}
\end{table}

% \begin{enumerate}
%   \item Exclusivity: $\operatorname{DSI}$ is an bijective (invertible) function, i.e., $\operatorname{M}: \mathcal{D} \twoheadrightarrow\!\!\!\!\!\!\mapsto \mathcal{I}$. % 从链接抄定义 \url{https://en.wikipedia.org/wiki/Injective_function} \url{https://en.wikipedia.org/wiki/Bijection}
%   \item Completeness:
%   \item Relevance: $$\forall d_i \in R(q, \operatorname{M})\;\text{and}\;\forall d_j \in D \setminus R(q, \operatorname{M}), d_j \leq_{q} d_i$$
%   $$\forall d_i, d_j \in R(q, \operatorname{M})\;\text{and}\;\operatorname{s}(q, d_j) \leq \operatorname{s}(q, d_i), d_j \leq_{q} d_i$$
%   % 定义 total order binary relation \leq_{q} \operatorname{R}(q,\operatorname{DSI}) <R, ≤q> a linear order set.
%   % https://www.vldb.org/pvldb/vol7/p745-liu.pdf
%   % total order https://en.wikipedia.org/wiki/Total_order
% \end{enumerate}







